A Survey on Intersectional Fairness in Machine Learning: Notions, Mitigation, and Challenges

The widespread adoption of Machine Learning systems, especially in more decision-critical applications such as criminal sentencing and bank loans, has led to increased concerns about fairness implications. Algorithms and metrics have been developed to mitigate and measure these discriminations. More recently, works have identified a more challenging form of bias called intersectional bias, which encompasses multiple sensitive attributes, such as race and gender, together. In this survey, we review the state-of-the-art in intersectional fairness. We present a taxonomy for intersectional notions of fairness and mitigation. Finally, we identify the key challenges and provide researchers with guidelines for future directions.

==> conclusion.tex <==
\section{Conclusion}

Intersectional fairness is a very important research problem in responsible AI. It has very unique challenges that reduce the effectiveness of traditional bias mitigation algorithms and the use of standard fairness metrics. In this work, we present a review of recent intersectional fairness works. We develop a taxonomy of bias mitigation methods, datasets available, specialized metrics and future directions. We hope this survey will organize the literature and help researchers by providing guidelines to open problems and challenges
